Wasserstein Gradient Flows for Scalable and Regularized Barycenter Computation

Wasserstein barycenters provide a principled approach for aggregating probability measures, while preserving the geometry of their ambient space. Existing discrete methods are not because as they assume access to the complete set of samples from the input measures. Meanwhile, neural network approaches do scale well, but rely on complex optimization problems and cannot easily incorporate label information. We address these limitations through gradient flows in the space of probability measures. Through time discretization, we achieve a scalable algorithm that i) relies on mini-batch optimal transport, ii) accepts modular regularization through task-aware functions, and iii) seamlessly integrates supervised information into the ground-cost. We empirically validate our approach on domain adaptation benchmarks that span computer vision, neuroscience, and chemical engineering. Our method establishes a new state-of-the-art Wasserstein barycenter solver, with labeled barycenters consistently outperforming unlabeled ones. Our code at https://github.com/SigmaNova/barycentric-gradient-flows

==> content/fig-sup-unsup.tex <==
\begin{figure*}[!b]
    \centering
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\linewidth]{Figures/unregularized_unlabeled_barycenter.pdf}
        \caption{Unsupervised}
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\linewidth]{Figures/regularized_unlabeled_barycenter.pdf}
        \caption{Unsupervised}
    \end{subfigure}\hfill %\\
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\linewidth]{Figures/unregularized_labeled_barycenter.pdf}
        \caption{Supervised}
    \end{subfigure}\hfill
    \begin{subfigure}{0.24\linewidth}
        \includegraphics[width=\linewidth]{Figures/regularized_labeled_barycenter.pdf}
        \caption{Supervised}
    \end{subfigure}\hfill
    \caption{t-SNE embeddings of unsupervised (a, b) and supervised (c, d) barycenters. While it is possible to group some samples according their pseudo-labels based on $\mathbb{U}$, the task is in general difficult. For the supervised case, the interaction energy is able to make classes more separable (d, in comparison to c).}
    \label{fig:vis}
\end{figure*}
